Dynamic Decision Frequency with Continuous Options

In classic reinforcement learning algorithms, agents make decisions at discrete and fixed time intervals. The duration between decisions becomes a crucial hyperparameter, as setting it too short may increase the problem's difficulty by requiring the agent to make numerous decisions to achieve its goal while setting it too long can result in the agent losing control over the system. However, physical systems do not necessarily require a constant control frequency, and for learning agents, it is often preferable to operate with a low frequency when possible and a high frequency when necessary. We propose a framework called Continuous-Time Continuous-Options (CTCO), where the agent chooses options as sub-policies of variable durations. These options are time-continuous and can interact with the system at any desired frequency providing a smooth change of actions. We demonstrate the effectiveness of CTCO by comparing its performance to classical RL and temporal-abstraction RL methods on simulated continuous control tasks with various action-cycle times. We show that our algorithm's performance is not affected by the choice of environment interaction frequency. Furthermore, we demonstrate the efficacy of CTCO in facilitating exploration in a real-world visual reaching task for a 7 DOF robotic arm with sparse rewards.

==> figures/freq_analysis_.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{gray}{RGB}{128,128,128}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{groupplot}[height=6cm,
width=6cm,group style={group size=3 by 1}]
\nextgroupplot[
log basis x={10},
tick align=outside,
tick pos=left,
title={Point mass},
x grid style={gray},
xlabel={Frequency (Hz) },
xmajorgrids,
xmin=20, xmax=1000,
xmode=log,
xtick style={color=black},
xtick={20,70,120,170,220,270,320,370,420,470,520,570,620,670,720,770,820,870,920,970},
xticklabels={,,\(\displaystyle {1.2\times10^{2}}\),,,,,,,,,,,,,,,,,},
y grid style={gray},
ylabel={Average discounted Return},
ymajorgrids,
ymin=-0.06186502549618, ymax=1.23710992426132,
ytick style={color=black}
]
\path [draw=steelblue31119180, semithick]
(axis cs:50,1.02523928167471)
--(axis cs:50,1.17806560836326);

\path [draw=steelblue31119180, semithick]
(axis cs:100,1.02183523937363)
--(axis cs:100,1.17109838133443);

\path [draw=steelblue31119180, semithick]
(axis cs:250,1.01467933448695)
--(axis cs:250,1.16491653467319);

\path [draw=steelblue31119180, semithick]
(axis cs:500,1.01178414431315)
--(axis cs:500,1.16658791967332);

\path [draw=darkorange25512714, semithick]
(axis cs:50,0.715246494224489)
--(axis cs:50,0.969003405699828);

\path [draw=darkorange25512714, semithick]
(axis cs:100,0.424100174501986)
--(axis cs:100,0.743288561375216);

\path [draw=darkorange25512714, semithick]
(axis cs:250,0.00223467726583378)
--(axis cs:250,0.0674244200659924);

\path [draw=darkorange25512714, semithick]
(axis cs:500,-0.00282070959811165)
--(axis cs:500,0.04153272130003);

\path [draw=forestgreen4416044, semithick]
(axis cs:50,0.78579748674878)
--(axis cs:50,1.01540677974553);

\path [draw=forestgreen4416044, semithick]
(axis cs:100,0.474622321969186)
--(axis cs:100,0.792401365339825);

\path [draw=forestgreen4416044, semithick]
(axis cs:250,0.316349901138162)
--(axis cs:250,0.619323970873308);

\path [draw=forestgreen4416044, semithick]
(axis cs:500,0.428147880193521)
--(axis cs:500,0.778973158192162);

\path [draw=crimson2143940, semithick]
(axis cs:50,0.433666860009722)
--(axis cs:50,0.650105092277152);

\path [draw=crimson2143940, semithick]
(axis cs:100,0.371894316640482)
--(axis cs:100,0.61469452846539);

\path [draw=crimson2143940, semithick]
(axis cs:250,0.181231797726136)
--(axis cs:250,0.4186103947281);

\path [draw=crimson2143940, semithick]
(axis cs:500,0.173418998999821)
--(axis cs:500,0.467818819363497);

\addplot [semithick, steelblue31119180, mark=*, mark size=3, mark options={solid}]
table {%
50 1.10165244501898
100 1.09646681035403
250 1.08979793458007
500 1.08918603199324
};
\addplot [semithick, darkorange25512714, mark=square*, mark size=3, mark options={solid}]
table {%
50 0.842124949962159
100 0.583694367938601
250 0.0348295486659131
500 0.0193560058509592
};
\addplot [semithick, forestgreen4416044, mark=triangle*, mark size=3, mark options={solid}]
table {%
50 0.900602133247157
100 0.633511843654506
250 0.467836936005735
500 0.603560519192841
};
\addplot [semithick, crimson2143940, mark=triangle*, mark size=3, mark options={solid,rotate=180}]
table {%
50 0.541885976143437
100 0.493294422552936
250 0.299921096227118
500 0.320618909181659
};

\nextgroupplot[
log basis x={10},
tick align=outside,
tick pos=left,
title={Cheetah},
x grid style={gray},
xlabel={Frequency (Hz) },
xmajorgrids,
xmin=20, xmax=1000,
xmode=log,
xtick style={color=black},
xtick={20,70,120,170,220,270,320,370,420,470,520,570,620,670,720,770,820,870,920,970},
xticklabels={,,\(\displaystyle {1.2\times10^{2}}\),,,,,,,,,,,,,,,,,},
y grid style={gray},
ylabel={Average discounted Return},
ymajorgrids,
ymin=-0.0222769487570324, ymax=1.2058371400195,
ytick style={color=black}
]
\path [draw=steelblue31119180, semithick]
(axis cs:50,0.616534140252482)
--(axis cs:50,0.666814951786582);

\path [draw=steelblue31119180, semithick]
(axis cs:100,0.622854146279241)
--(axis cs:100,0.673413444193218);

\path [draw=steelblue31119180, semithick]
(axis cs:250,0.643121087010499)
--(axis cs:250,0.690390274134348);

\path [draw=steelblue31119180, semithick]
(axis cs:500,0.640264582108639)
--(axis cs:500,0.68679283155123);

\path [draw=darkorange25512714, semithick]
(axis cs:50,0.980334548070098)
--(axis cs:50,1.13144285393518);

\path [draw=darkorange25512714, semithick]
(axis cs:100,0.101903986010229)
--(axis cs:100,0.235413266020942);

\path [draw=darkorange25512714, semithick]
(axis cs:250,0.0335464189146283)
--(axis cs:250,0.0684458444024629);

\path [draw=darkorange25512714, semithick]
(axis cs:500,0.051201451492302)
--(axis cs:500,0.0834695051988473);

\path [draw=forestgreen4416044, semithick]
(axis cs:50,0.996631849461582)
--(axis cs:50,1.10542969701686);

\path [draw=forestgreen4416044, semithick]
(axis cs:100,1.08081869322211)
--(axis cs:100,1.15001377234784);

\path [draw=forestgreen4416044, semithick]
(axis cs:250,0.578711780275264)
--(axis cs:250,0.899831910158835);

\path [draw=forestgreen4416044, semithick]
(axis cs:500,0.126040872888543)
--(axis cs:500,0.196272729804076);

\path [draw=crimson2143940, semithick]
(axis cs:50,0.55847795641818)
--(axis cs:50,0.600458664919401);

\path [draw=crimson2143940, semithick]
(axis cs:100,0.454099673266191)
--(axis cs:100,0.497933445419504);

\path [draw=crimson2143940, semithick]
(axis cs:250,0.318132178958944)
--(axis cs:250,0.373941045573702);

\path [draw=crimson2143940, semithick]
(axis cs:500,0.200202508365127)
--(axis cs:500,0.285047932729988);

\addplot [semithick, steelblue31119180, mark=*, mark size=3, mark options={solid}]
table {%
50 0.641674546019532
100 0.64813379523623
250 0.666755680572423
500 0.663528706829935
};
\addplot [semithick, darkorange25512714, mark=square*, mark size=3, mark options={solid}]
table {%
50 1.05588870100264
100 0.168658626015586
250 0.0509961316585456
500 0.0673354783455746
};
\addplot [semithick, forestgreen4416044, mark=triangle*, mark size=3, mark options={solid}]
table {%
50 1.05103077323922
100 1.11541623278498
250 0.739271845217049
500 0.161156801346309
};
\addplot [semithick, crimson2143940, mark=triangle*, mark size=3, mark options={solid,rotate=180}]
table {%
50 0.57946831066879
100 0.476016559342847
250 0.346036612266323
500 0.242625220547558
};

\nextgroupplot[
log basis x={10},
tick align=outside,
tick pos=left,
title={Ball in cup},
x grid style={gray},
xlabel={Frequency (Hz) },
xmajorgrids,
xmin=20, xmax=1000,
xmode=log,
xtick style={color=black},
xtick={20,70,120,170,220,270,320,370,420,470,520,570,620,670,720,770,820,870,920,970},
xticklabels={,,\(\displaystyle {1.2\times10^{2}}\),,,,,,,,,,,,,,,,,},
y grid style={gray},
ylabel={Average discounted Return},
ymajorgrids,
ymin=0.042345569988419, ymax=2.117163768253,
ytick style={color=black}
]
\path [draw=steelblue31119180, semithick]
(axis cs:50,1.48019566270448)
--(axis cs:50,1.72313929255879);

\path [draw=steelblue31119180, semithick]
(axis cs:100,1.40206212654188)
--(axis cs:100,1.66386139218716);

\path [draw=steelblue31119180, semithick]
(axis cs:250,1.42236856753808)
--(axis cs:250,1.69861783360247);

\path [draw=steelblue31119180, semithick]
(axis cs:500,1.42306986234475)
--(axis cs:500,1.72096554486617);

\path [draw=darkorange25512714, semithick]
(axis cs:50,1.82360148947508)
--(axis cs:50,1.97607001737588);

\path [draw=darkorange25512714, semithick]
(axis cs:100,0.210557110709847)
--(axis cs:100,0.577027978890425);

\path [draw=darkorange25512714, semithick]
(axis cs:250,0.141479125626021)
--(axis cs:250,0.437717461860644);

\path [draw=darkorange25512714, semithick]
(axis cs:500,0.136655488091355)
--(axis cs:500,0.439220562340457);

\path [draw=forestgreen4416044, semithick]
(axis cs:50,1.81036567613417)
--(axis cs:50,1.98707701333212);

\path [draw=forestgreen4416044, semithick]
(axis cs:100,1.82242978062131)
--(axis cs:100,2.02285385015007);

\path [draw=forestgreen4416044, semithick]
(axis cs:250,1.71806612756929)
--(axis cs:250,1.98656006729259);

\path [draw=forestgreen4416044, semithick]
(axis cs:500,0.611703076840587)
--(axis cs:500,1.05106208292012);

\path [draw=crimson2143940, semithick]
(axis cs:50,0.769066928205708)
--(axis cs:50,1.07765410976612);

\path [draw=crimson2143940, semithick]
(axis cs:100,0.874030146030603)
--(axis cs:100,1.20298996831265);

\path [draw=crimson2143940, semithick]
(axis cs:250,0.550948611237313)
--(axis cs:250,0.949406064785105);

\path [draw=crimson2143940, semithick]
(axis cs:500,0.302077963884254)
--(axis cs:500,0.867564808929188);

\addplot [semithick, steelblue31119180, mark=*, mark size=3, mark options={solid}]
table {%
50 1.60166747763164
100 1.53296175936452
250 1.56049320057028
500 1.57201770360546
};
\addplot [semithick, darkorange25512714, mark=square*, mark size=3, mark options={solid}]
table {%
50 1.89983575342548
100 0.393792544800136
250 0.289598293743333
500 0.287938025215906
};
\addplot [semithick, forestgreen4416044, mark=triangle*, mark size=3, mark options={solid}]
table {%
50 1.89872134473314
100 1.92264181538569
250 1.85231309743094
500 0.831382579880355
};
\addplot [semithick, crimson2143940, mark=triangle*, mark size=3, mark options={solid,rotate=180}]
table {%
50 0.923360518985912
100 1.03851005717162
250 0.750177338011209
500 0.584821386406721
};
\end{groupplot}

\end{tikzpicture}


==> figures/freq_plot_tikz.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{gray}{RGB}{128,128,128}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{groupplot}[group style={group size=3 by 1}]
\nextgroupplot[
log basis x={10},
tick align=outside,
tick pos=left,
title={Mountain\_car},
x grid style={gray},
xlabel={Frequency (Hz) },
xmajorgrids,
xmin=10, xmax=1000,
xmode=log,
xtick style={color=black},
xtick={10,60,110,160,210,260,310,360,410,460,510,560,610,660,710,760,810,860,910,960},
xticklabels={\(\displaystyle {10^{1}}\),,\(\displaystyle {1.1\times10^{2}}\),,,,,,,,,,,,,,,,,},
y grid style={gray},
ylabel={Average discounted Return},
ymajorgrids,
ymin=-0.16120406967237, ymax=0.777637105473349,
ytick style={color=black}
]
\path [draw=steelblue31119180, semithick]
(axis cs:20,0.587121952972405)
--(axis cs:20,0.641584611022774);

\path [draw=steelblue31119180, semithick]
(axis cs:40,0.529054692513894)
--(axis cs:40,0.655064800937314);

\path [draw=steelblue31119180, semithick]
(axis cs:80,0.595377689497303)
--(axis cs:80,0.63336070435591);

\path [draw=steelblue31119180, semithick]
(axis cs:160,0.581786792552312)
--(axis cs:160,0.629981928671027);

\path [draw=steelblue31119180, semithick]
(axis cs:320,0.605917270650235)
--(axis cs:320,0.632822956571992);

\path [draw=darkorange25512714, semithick]
(axis cs:20,0.6042475423715)
--(axis cs:20,0.734962506603089);

\path [draw=darkorange25512714, semithick]
(axis cs:40,0.267381006416504)
--(axis cs:40,0.519231598791823);

\path [draw=darkorange25512714, semithick]
(axis cs:80,-0.0271167499214372)
--(axis cs:80,0.0613150638257736);

\path [draw=darkorange25512714, semithick]
(axis cs:160,-0.0491808421866482)
--(axis cs:160,0.100600869564746);

\path [draw=darkorange25512714, semithick]
(axis cs:320,-0.11852947080211)
--(axis cs:320,-0.0198375397272562);

\path [draw=forestgreen4416044, semithick]
(axis cs:320,0.176030739790234)
--(axis cs:320,0.462578288749055);

\path [draw=forestgreen4416044, semithick]
(axis cs:160,0.614278087454644)
--(axis cs:160,0.729224502942131);

\path [draw=forestgreen4416044, semithick]
(axis cs:80,0.703466176475923)
--(axis cs:80,0.705423123012839);

\path [draw=forestgreen4416044, semithick]
(axis cs:40,0.699617021252979)
--(axis cs:40,0.703194633714383);

\path [draw=forestgreen4416044, semithick]
(axis cs:20,0.636814742994851)
--(axis cs:20,0.651460704612048);

\path [draw=crimson2143940, semithick]
(axis cs:320,-0.00263778739984525)
--(axis cs:320,-0.00136956214960252);

\path [draw=crimson2143940, semithick]
(axis cs:160,0.0651054457558067)
--(axis cs:160,0.0706578499629347);

\path [draw=crimson2143940, semithick]
(axis cs:80,0.225178493040936)
--(axis cs:80,0.245281666573767);

\path [draw=crimson2143940, semithick]
(axis cs:40,0.430246574804511)
--(axis cs:40,0.437148176763732);

\path [draw=crimson2143940, semithick]
(axis cs:20,0.578420562121897)
--(axis cs:20,0.585296047435621);

\addplot [semithick, steelblue31119180, mark=*, mark size=3, mark options={solid}]
table {%
20 0.614353281997589
40 0.592059746725604
80 0.614369196926607
160 0.605884360611669
320 0.619370113611114
};
\addplot [semithick, darkorange25512714, mark=square*, mark size=3, mark options={solid}]
table {%
20 0.669605024487295
40 0.393306302604163
80 0.0170991569521682
160 0.025710013689049
320 -0.0691835052646833
};
\addplot [semithick, forestgreen4416044, mark=triangle*, mark size=3, mark options={solid}]
table {%
320 0.319304514269645
160 0.671751295198387
80 0.704444649744381
40 0.701405827483681
20 0.64413772380345
};
\addplot [semithick, crimson2143940, mark=triangle*, mark size=3, mark options={solid,rotate=180}]
table {%
320 -0.00200367477472389
160 0.0678816478593707
80 0.235230079807352
40 0.433697375784121
20 0.581858304778759
};

\nextgroupplot[
log basis x={10},
tick align=outside,
tick pos=left,
title={Half\_cheetah},
x grid style={gray},
xlabel={Frequency (Hz) },
xmajorgrids,
xmin=10, xmax=1000,
xmode=log,
xtick style={color=black},
xtick={10,60,110,160,210,260,310,360,410,460,510,560,610,660,710,760,810,860,910,960},
xticklabels={\(\displaystyle {10^{1}}\),,\(\displaystyle {1.1\times10^{2}}\),,,,,,,,,,,,,,,,,},
y grid style={gray},
ylabel={Average discounted Return},
ymajorgrids,
ymin=-2.9031256294957, ymax=9.33786066023913,
ytick style={color=black}
]
\path [draw=steelblue31119180, semithick]
(axis cs:20,2.99038928128788)
--(axis cs:20,3.68416613814898);

\path [draw=steelblue31119180, semithick]
(axis cs:80,2.74827372139009)
--(axis cs:80,3.6993631627545);

\path [draw=steelblue31119180, semithick]
(axis cs:320,3.17082782706024)
--(axis cs:320,4.01639283877666);

\path [draw=darkorange25512714, semithick]
(axis cs:20,5.38611477324999)
--(axis cs:20,6.60466660243618);

\path [draw=darkorange25512714, semithick]
(axis cs:40,6.40231115103071)
--(axis cs:40,8.13140171216411);

\path [draw=darkorange25512714, semithick]
(axis cs:80,-1.19919660405039)
--(axis cs:80,0.296552334268377);

\path [draw=darkorange25512714, semithick]
(axis cs:160,-2.29223473270532)
--(axis cs:160,-1.13379178157254);

\path [draw=darkorange25512714, semithick]
(axis cs:320,-2.34671716178048)
--(axis cs:320,-0.974204332841093);

\path [draw=forestgreen4416044, semithick]
(axis cs:320,0.411200837200801)
--(axis cs:320,2.96786793871738);

\path [draw=forestgreen4416044, semithick]
(axis cs:160,7.80049088171843)
--(axis cs:160,8.78145219252391);

\path [draw=forestgreen4416044, semithick]
(axis cs:80,3.78825570968927)
--(axis cs:80,5.60451764389148);

\path [draw=forestgreen4416044, semithick]
(axis cs:40,3.31524408906355)
--(axis cs:40,4.50498295011329);

\path [draw=forestgreen4416044, semithick]
(axis cs:20,1.72865200409934)
--(axis cs:20,2.97925796810196);

\path [draw=crimson2143940, semithick]
(axis cs:320,-0.0334990968604457)
--(axis cs:320,-0.00314724608821284);

\path [draw=crimson2143940, semithick]
(axis cs:160,0.0816904056770156)
--(axis cs:160,0.129934231200109);

\path [draw=crimson2143940, semithick]
(axis cs:80,0.578526602604029)
--(axis cs:80,0.715275424444935);

\path [draw=crimson2143940, semithick]
(axis cs:40,1.78551391515616)
--(axis cs:40,2.32115061475279);

\path [draw=crimson2143940, semithick]
(axis cs:20,3.55799885860813)
--(axis cs:20,5.18666547091447);

\addplot [semithick, steelblue31119180, mark=*, mark size=3, mark options={solid}]
table {%
20 3.33727770971843
80 3.22381844207229
320 3.59361033291845
};
\addplot [semithick, darkorange25512714, mark=square*, mark size=3, mark options={solid}]
table {%
20 5.99539068784308
40 7.26685643159741
80 -0.451322134891007
160 -1.71301325713893
320 -1.66046074731079
};
\addplot [semithick, forestgreen4416044, mark=triangle*, mark size=3, mark options={solid}]
table {%
320 1.68953438795909
160 8.29097153712117
80 4.69638667679038
40 3.91011351958842
20 2.35395498610065
};
\addplot [semithick, crimson2143940, mark=triangle*, mark size=3, mark options={solid,rotate=180}]
table {%
320 -0.0183231714743293
160 0.105812318438562
80 0.646901013524482
40 2.05333226495447
20 4.3723321647613
};

\nextgroupplot[
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.09,0.5)},
  anchor=west,
  draw=lightgray204
},
log basis x={10},
tick align=outside,
tick pos=left,
title={Ball\_in\_cup},
x grid style={gray},
xlabel={Frequency (Hz) },
xmajorgrids,
xmin=10, xmax=1000,
xmode=log,
xtick style={color=black},
xtick={10,60,110,160,210,260,310,360,410,460,510,560,610,660,710,760,810,860,910,960},
xticklabels={\(\displaystyle {10^{1}}\),,\(\displaystyle {1.1\times10^{2}}\),,,,,,,,,,,,,,,,,},
y grid style={gray},
ylabel={Average discounted Return},
ymajorgrids,
ymin=-0.10218709905987, ymax=2.15751159493258,
ytick style={color=black}
]
\path [draw=steelblue31119180, semithick]
(axis cs:50,1.73743461533353)
--(axis cs:50,1.9032659204745);

\path [draw=steelblue31119180, semithick]
(axis cs:100,1.70855878388644)
--(axis cs:100,1.92634066619775);

\path [draw=steelblue31119180, semithick]
(axis cs:250,1.57042659038418)
--(axis cs:250,1.80048739261449);

\path [draw=steelblue31119180, semithick]
(axis cs:500,1.53085296005359)
--(axis cs:500,1.80524176717498);

\path [draw=darkorange25512714, semithick]
(axis cs:50,1.68070069416785)
--(axis cs:50,1.94899973414983);

\path [draw=darkorange25512714, semithick]
(axis cs:100,0.274521504695095)
--(axis cs:100,0.714257909326564);

\path [draw=darkorange25512714, semithick]
(axis cs:250,0.170117960450513)
--(axis cs:250,0.632229675104459);

\path [draw=darkorange25512714, semithick]
(axis cs:500,0.0985361417776904)
--(axis cs:500,0.415591401374054);

\path [draw=forestgreen4416044, semithick]
(axis cs:500,0.48580699184751)
--(axis cs:500,1.04553816631541);

\path [draw=forestgreen4416044, semithick]
(axis cs:250,1.67528522017869)
--(axis cs:250,1.9519174967968);

\path [draw=forestgreen4416044, semithick]
(axis cs:100,1.86961307342919)
--(axis cs:100,2.01612712197458);

\path [draw=forestgreen4416044, semithick]
(axis cs:50,1.87494367799868)
--(axis cs:50,2.05479801793293);

\path [draw=crimson2143940, semithick]
(axis cs:500,0.000526477939786733)
--(axis cs:500,0.0025009568860456);

\path [draw=crimson2143940, semithick]
(axis cs:250,0.00396847786042462)
--(axis cs:250,0.02271698731196);

\path [draw=crimson2143940, semithick]
(axis cs:100,0.0480307518043331)
--(axis cs:100,0.104750485226193);

\path [draw=crimson2143940, semithick]
(axis cs:50,0.198108307877657)
--(axis cs:50,0.369572978036527);

\addplot [semithick, steelblue31119180, mark=*, mark size=3, mark options={solid}]
table {%
50 1.82035026790401
100 1.81744972504209
250 1.68545699149933
500 1.66804736361428
};
\addlegendentry{DAC}
\addplot [semithick, darkorange25512714, mark=square*, mark size=3, mark options={solid}]
table {%
50 1.81485021415884
100 0.494389707010829
250 0.401173817777486
500 0.257063771575872
};
\addlegendentry{DAC}
\addplot [semithick, forestgreen4416044, mark=triangle*, mark size=3, mark options={solid}]
table {%
500 0.765672579081459
250 1.81360135848774
100 1.94287009770189
50 1.9648708479658
};
\addlegendentry{DAC}
\addplot [semithick, crimson2143940, mark=triangle*, mark size=3, mark options={solid,rotate=180}]
table {%
500 0.00151371741291616
250 0.0133427325861923
100 0.076390618515263
50 0.283840642957092
};
\addlegendentry{DAC}
\end{groupplot}

\draw ({$(current bounding box.south west)!0.5!(current bounding box.south east)$}|-{$(current bounding box.south west)!0.98!(current bounding box.north west)$}) node[
  scale=0.6,
  anchor=north,
  text=black,
  rotate=0.0
]{Final performance of algorithms vs frequency};
\end{tikzpicture}


==> figures/legend.tex <==
\begin{tikzpicture}
\definecolor{red}{RGB}{214,39,40}
\definecolor{orange}{RGB}{255,127,14}
\definecolor{green}{RGB}{44,160,44}
\definecolor{gray}{RGB}{128,128,128}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{blue}{RGB}{31,119,180}

\begin{axis}[
height=2cm,
width=8cm,
hide axis,
xmin=10,
xmax=50,
ymin=0,
ymax=0.5,
legend columns=-1,
legend entries={{SAC}, {FiGAR-SAC}, {DAC-PPO}, {CTCO}},
legend style={at={(0.6,0.5)}, anchor=north, draw=none, font=\scriptsize, column sep=1ex, line width=2 pt},
]
		\addlegendimage{no markers, orange}
		\addlegendimage{no markers, green}
		\addlegendimage{no markers, red}
		\addlegendimage{no markers, blue}
\end{axis}
\end{tikzpicture}

==> figures/real_world_result.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{steelblue31119180}{RGB}{31,119,180}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{darkorange25512714}{RGB}{255,127,14}

\begin{axis}[
height=4.5cm,
tick align=outside,
tick pos=left,
title={\small Visual Reacher},
title style={yshift=-0.15cm},
unbounded coords=jump,
grid=both,
x grid style={darkgray176},
xlabel={\small Time (min)},
xmin=0, xmax=70,%xmax=103.95,
xtick style={color=white},
y grid style={darkgray176},
ylabel={\small $J^\tau_\pi(\theta)$},
ymin=-0.487422566295491, ymax=1.7, %ymax=2.62264349059552,
ytick style={color=white},
yticklabel style={font=\tiny, xshift=0.2cm},
xticklabel style={font=\tiny, yshift=0.1cm},
ylabel style={yshift=-0.6cm}
]
\path [draw=darkorange25512714, fill=darkorange25512714, opacity=0.3]
(axis cs:0,0)
--(axis cs:0,0)
--(axis cs:1,0)
--(axis cs:2,-0.0294188283423424)
--(axis cs:3,-0.0713142857142857)
--(axis cs:4,0)
--(axis cs:5,-0.0357614418687779)
--(axis cs:6,0)
--(axis cs:7,-0.0505589777470482)
--(axis cs:8,-0.105325714285714)
--(axis cs:9,-0.00096)
--(axis cs:10,-0.0625371428571429)
--(axis cs:11,-0.0223632413826789)
--(axis cs:12,-0.00658285714285714)
--(axis cs:13,0)
--(axis cs:14,0)
--(axis cs:15,0)
--(axis cs:16,-0.0394971428571429)
--(axis cs:17,-0.0209233445043691)
--(axis cs:18,-0.0872228571428571)
--(axis cs:19,-0.0256354423256736)
--(axis cs:20,-0.0109714285714286)
--(axis cs:21,-0.11136)
--(axis cs:22,-0.0318171428571429)
--(axis cs:23,0)
--(axis cs:24,0)
--(axis cs:25,-0.00576)
--(axis cs:26,-0.112519186428047)
--(axis cs:27,-0.05472)
--(axis cs:28,-0.143725714285714)
--(axis cs:29,-0.32688)
--(axis cs:30,-0.0280561811720156)
--(axis cs:31,-0.01056)
--(axis cs:32,0)
--(axis cs:33,-0.00447599608471225)
--(axis cs:34,-0.0197485714285714)
--(axis cs:35,-0.06336)
--(axis cs:36,0)
--(axis cs:37,0)
--(axis cs:38,-0.0208457142857143)
--(axis cs:39,-0.03936)
--(axis cs:40,0)
--(axis cs:41,-0.09696)
--(axis cs:42,-0.0252342857142857)
--(axis cs:43,-0.12672)
--(axis cs:44,-0.04233899596626)
--(axis cs:45,-0.0368682784251077)
--(axis cs:46,-0.0936303699826106)
--(axis cs:47,-0.09888)
--(axis cs:48,-0.05376)
--(axis cs:49,-0.0700472234815256)
--(axis cs:50,-0.00987428571428572)
--(axis cs:51,-0.12816)
--(axis cs:52,-0.102270150706895)
--(axis cs:53,-0.0150924620896831)
--(axis cs:54,-0.112115045369781)
--(axis cs:55,0)
--(axis cs:56,-0.0254739148102884)
--(axis cs:57,-0.0923447174894947)
--(axis cs:58,-0.121315855009874)
--(axis cs:59,-0.01248)
--(axis cs:60,-0.0120775674400977)
--(axis cs:61,0.00531908372478215)
--(axis cs:62,-0.0423372788825687)
--(axis cs:63,-0.0336)
--(axis cs:64,0)
--(axis cs:65,-0.02304)
--(axis cs:66,-0.122224237773989)
--(axis cs:67,-0.0417728515076719)
--(axis cs:68,-0.0758328554536365)
--(axis cs:69,-0.18384)
--(axis cs:70,-0.0216789047614009)
--(axis cs:71,-0.067901529175237)
--(axis cs:72,-0.00777314207569961)
--(axis cs:73,-0.0331725306022353)
--(axis cs:74,-0.0463665947642223)
--(axis cs:74,0.513033261430889)
--(axis cs:74,0.513033261430889)
--(axis cs:73,0.321172530602235)
--(axis cs:72,0.0377731420756996)
--(axis cs:71,0.339901529175237)
--(axis cs:70,0.198821761904258)
--(axis cs:69,0.56684)
--(axis cs:68,0.340975712596494)
--(axis cs:67,0.291772851507672)
--(axis cs:66,0.630795666345417)
--(axis cs:65,0.07104)
--(axis cs:64,0)
--(axis cs:63,0.1036)
--(axis cs:62,0.280051564596854)
--(axis cs:61,0.126680916275218)
--(axis cs:60,0.0966489960115262)
--(axis cs:59,0.03848)
--(axis cs:58,0.530458712152731)
--(axis cs:57,0.398344717489495)
--(axis cs:56,0.194616771953146)
--(axis cs:55,0)
--(axis cs:54,0.507543616798352)
--(axis cs:53,0.105092462089683)
--(axis cs:52,0.640555864992609)
--(axis cs:51,0.39516)
--(axis cs:50,0.0304457142857143)
--(axis cs:49,0.312047223481526)
--(axis cs:48,0.16576)
--(axis cs:47,0.30488)
--(axis cs:46,0.575916084268325)
--(axis cs:45,0.210868278425108)
--(axis cs:44,0.289196138823403)
--(axis cs:43,0.39072)
--(axis cs:42,0.0778057142857143)
--(axis cs:41,0.29896)
--(axis cs:40,0)
--(axis cs:39,0.12136)
--(axis cs:38,0.0642742857142857)
--(axis cs:37,0)
--(axis cs:36,0)
--(axis cs:35,0.19536)
--(axis cs:34,0.0608914285714286)
--(axis cs:33,0.0404759960847122)
--(axis cs:32,0)
--(axis cs:31,0.03256)
--(axis cs:30,0.170913324029158)
--(axis cs:29,1.00788)
--(axis cs:28,0.443154285714286)
--(axis cs:27,0.16872)
--(axis cs:26,0.386804900713761)
--(axis cs:25,0.01776)
--(axis cs:24,0)
--(axis cs:23,0)
--(axis cs:22,0.0981028571428572)
--(axis cs:21,0.34336)
--(axis cs:20,0.0338285714285714)
--(axis cs:19,0.273635442325674)
--(axis cs:18,0.268937142857143)
--(axis cs:17,0.192923344504369)
--(axis cs:16,0.121782857142857)
--(axis cs:15,0)
--(axis cs:14,0)
--(axis cs:13,0)
--(axis cs:12,0.0202971428571429)
--(axis cs:11,0.134363241382679)
--(axis cs:10,0.192822857142857)
--(axis cs:9,0.00296)
--(axis cs:8,0.324754285714286)
--(axis cs:7,0.330558977747048)
--(axis cs:6,0)
--(axis cs:5,0.161761441868778)
--(axis cs:4,0)
--(axis cs:3,0.219885714285714)
--(axis cs:2,0.171133114056628)
--(axis cs:1,0)
--(axis cs:0,0)
--cycle;

\path [draw=steelblue31119180, fill=steelblue31119180, opacity=0.3]
(axis cs:0,0.3552)
--(axis cs:0,-0.1152)
--(axis cs:1,-0.0916114285714286)
--(axis cs:2,0)
--(axis cs:3,0.0350810994311004)
--(axis cs:4,-0.0276437041479183)
--(axis cs:5,-0.0277646908123496)
--(axis cs:6,-0.0180547218683375)
--(axis cs:7,-0.0383357438168104)
--(axis cs:8,-0.0450544152887874)
--(axis cs:9,-0.0329142857142857)
--(axis cs:10,-0.0454713833235189)
--(axis cs:11,-0.0422092683201354)
--(axis cs:12,-0.0646353997395509)
--(axis cs:13,-0.0114428556550718)
--(axis cs:14,-0.12771698346858)
--(axis cs:15,-0.0107330785350345)
--(axis cs:16,-0.148628131477905)
--(axis cs:17,-0.0553868961662797)
--(axis cs:18,-0.27648)
--(axis cs:19,-0.00642578900531837)
--(axis cs:20,0.0200467741784836)
--(axis cs:21,-0.0792695694192709)
--(axis cs:22,-0.00305477358955619)
--(axis cs:23,-0.0745500602366156)
--(axis cs:24,-0.0237848349677899)
--(axis cs:25,-0.0190040689579264)
--(axis cs:26,-0.0656860128099755)
--(axis cs:27,-0.00371402389579231)
--(axis cs:28,-0.253470972715073)
--(axis cs:29,-0.12308003362299)
--(axis cs:30,0.0675921188175372)
--(axis cs:31,0.0725075484938679)
--(axis cs:32,-0.0143776845324387)
--(axis cs:33,0.0121938751325951)
--(axis cs:34,-0.0535497949790437)
--(axis cs:35,-0.0375425346136003)
--(axis cs:36,-0.27132822308648)
--(axis cs:37,-0.0324326490776031)
--(axis cs:38,-0.037193620161161)
--(axis cs:39,-0.271363213186103)
--(axis cs:40,0.0600002864516659)
--(axis cs:41,0.25224868318359)
--(axis cs:42,-0.185158724505402)
--(axis cs:43,0.00879634980157984)
--(axis cs:44,0.069512479689798)
--(axis cs:45,0.074556051634407)
--(axis cs:46,0.0271834834162258)
--(axis cs:47,0.127087443861187)
--(axis cs:48,0.220151239183473)
--(axis cs:49,-0.346055927345899)
--(axis cs:50,0.044498774014793)
--(axis cs:51,-0.019155337440467)
--(axis cs:52,0.144226480283194)
--(axis cs:53,-0.118406698472381)
--(axis cs:54,0.239810149995321)
--(axis cs:55,0.116211118565659)
--(axis cs:56,-0.0974150106359321)
--(axis cs:57,-0.0580892789024388)
--(axis cs:58,-0.0430990139586424)
--(axis cs:59,0.00871647464516889)
--(axis cs:60,0.228744682787363)
--(axis cs:61,0.11937834376615)
--(axis cs:62,0.0950318764421488)
--(axis cs:63,-0.14342194685172)
--(axis cs:64,0.304141840938069)
--(axis cs:65,0.0987243599037847)
--(axis cs:66,0.198679364679586)
--(axis cs:67,0.328510768968075)
--(axis cs:68,0.38997736587645)
--(axis cs:69,0.244135440732641)
--(axis cs:70,0.861148986072571)
--(axis cs:71,0.295972613457233)
--(axis cs:72,0.578412760996321)
--(axis cs:73,0.418943657786111)
--(axis cs:74,0.664413400862283)
--(axis cs:75,0.445150057175919)
--(axis cs:76,0.603627218311839)
--(axis cs:77,0.326173119314387)
--(axis cs:78,0.445886231499731)
--(axis cs:79,0.444833257129979)
--(axis cs:80,0.187366408262906)
--(axis cs:81,0.114890936283025)
--(axis cs:82,0.258556085947985)
--(axis cs:83,0.137261393620034)
--(axis cs:84,0.38410226969006)
--(axis cs:85,0.660084396087113)
--(axis cs:86,0.326189835230694)
--(axis cs:87,0.507925955513421)
--(axis cs:88,0.204948730474182)
--(axis cs:89,0.369679666212612)
--(axis cs:90,0.420384664063188)
--(axis cs:91,0.153839864366446)
--(axis cs:92,0.82681924112191)
--(axis cs:93,0.774619442601546)
--(axis cs:94,0.424651320957037)
--(axis cs:95,0.382723148354068)
--(axis cs:96,0.608576537981723)
--(axis cs:97,0.294078691952235)
--(axis cs:98,0.53988467806363)
--(axis cs:99,0.825728726229804)
--(axis cs:99,2.28798555948448)
--(axis cs:99,2.28798555948448)
--(axis cs:98,1.27725817907923)
--(axis cs:97,1.95992130804776)
--(axis cs:96,2.05656631916113)
--(axis cs:95,2.48127685164593)
--(axis cs:94,2.10563439332868)
--(axis cs:93,2.41438055739845)
--(axis cs:92,1.83375218744952)
--(axis cs:91,2.01916013563355)
--(axis cs:90,2.4413296216511)
--(axis cs:89,1.80832033378739)
--(axis cs:88,2.2407655552401)
--(axis cs:87,1.18507404448658)
--(axis cs:86,1.96181016476931)
--(axis cs:85,1.24191560391289)
--(axis cs:84,1.43575487316708)
--(axis cs:83,1.65231003495139)
--(axis cs:82,2.22644391405202)
--(axis cs:81,0.981680492288403)
--(axis cs:80,2.00863359173709)
--(axis cs:79,1.78259531429859)
--(axis cs:78,1.29511376850027)
--(axis cs:77,1.72411259497133)
--(axis cs:76,2.02237278168816)
--(axis cs:75,2.0131356571098)
--(axis cs:74,1.93958659913772)
--(axis cs:73,1.90219919935675)
--(axis cs:72,2.03458723900368)
--(axis cs:71,1.18402738654277)
--(axis cs:70,2.16785101392743)
--(axis cs:69,1.16157884498164)
--(axis cs:68,1.89302263412355)
--(axis cs:67,1.62006065960335)
--(axis cs:66,1.72232063532041)
--(axis cs:65,1.47041849723907)
--(axis cs:64,1.58185815906193)
--(axis cs:63,1.80742194685172)
--(axis cs:62,1.59696812355785)
--(axis cs:61,1.02690737051956)
--(axis cs:60,1.93225531721264)
--(axis cs:59,0.889569239640545)
--(axis cs:58,1.93409901395864)
--(axis cs:57,2.01580356461672)
--(axis cs:56,1.61141501063593)
--(axis cs:55,1.31350316714863)
--(axis cs:54,1.73118985000468)
--(axis cs:53,1.68297812704381)
--(axis cs:52,1.32077351971681)
--(axis cs:51,1.03744105172618)
--(axis cs:50,1.76850122598521)
--(axis cs:49,1.61348449877447)
--(axis cs:48,1.10984876081653)
--(axis cs:47,0.656912556138813)
--(axis cs:46,0.221816516583774)
--(axis cs:45,1.17572966265131)
--(axis cs:44,1.8884875203102)
--(axis cs:43,1.27463222162699)
--(axis cs:42,1.6721587245054)
--(axis cs:41,1.20717988824498)
--(axis cs:40,1.60999971354833)
--(axis cs:39,2.09879178461467)
--(axis cs:38,0.405193620161161)
--(axis cs:37,0.642718363363317)
--(axis cs:36,1.37832822308648)
--(axis cs:35,0.759828248899315)
--(axis cs:34,1.11754979497904)
--(axis cs:33,0.84152041058169)
--(axis cs:32,1.18537768453244)
--(axis cs:31,0.842921022934703)
--(axis cs:30,1.24640788118246)
--(axis cs:29,0.520794319337275)
--(axis cs:28,1.00147097271507)
--(axis cs:27,0.216285452467221)
--(axis cs:26,0.980686012809976)
--(axis cs:25,0.901289783243641)
--(axis cs:24,0.16178483496779)
--(axis cs:23,0.389978631665187)
--(axis cs:22,0.777054773589556)
--(axis cs:21,0.623269569419271)
--(axis cs:20,0.399953225821516)
--(axis cs:19,0.694425789005318)
--(axis cs:18,0.85248)
--(axis cs:17,0.606244039023422)
--(axis cs:16,0.651628131477905)
--(axis cs:15,0.10444736424932)
--(axis cs:14,0.86971698346858)
--(axis cs:13,0.125728569940786)
--(axis cs:12,0.446635399739551)
--(axis cs:11,0.135923554034421)
--(axis cs:10,0.183471383323519)
--(axis cs:9,0.101485714285714)
--(axis cs:8,0.246197272431645)
--(axis cs:7,0.135192886673953)
--(axis cs:6,0.0920547218683375)
--(axis cs:5,0.22976469081235)
--(axis cs:4,0.423357989862204)
--(axis cs:3,0.347776043426043)
--(axis cs:2,0)
--(axis cs:1,0.282468571428571)
--(axis cs:0,0.3552)
--cycle;

\addplot [semithick, darkorange25512714]
table {%
0 0
1 0
2 0.0708571428571429
3 0.0742857142857143
4 0
5 0.063
6 0
7 0.14
8 0.109714285714286
9 0.001
10 0.0651428571428571
11 0.056
12 0.00685714285714286
13 0
14 0
15 0
16 0.0411428571428571
17 0.086
18 0.0908571428571428
19 0.124
20 0.0114285714285714
21 0.116
22 0.0331428571428571
23 0
24 0
25 0.006
26 0.137142857142857
27 0.057
28 0.149714285714286
29 0.3405
30 0.0714285714285714
31 0.011
32 0
33 0.018
34 0.0205714285714286
35 0.066
36 0
37 0
38 0.0217142857142857
39 0.041
40 0
41 0.101
42 0.0262857142857143
43 0.132
44 0.123428571428571
45 0.087
46 0.241142857142857
47 0.103
48 0.056
49 0.121
50 0.0102857142857143
51 0.1335
52 0.269142857142857
53 0.045
54 0.197714285714286
55 0
56 0.0845714285714286
57 0.153
58 0.204571428571429
59 0.013
60 0.0422857142857143
61 0.066
62 0.118857142857143
63 0.035
64 0
65 0.024
66 0.254285714285714
67 0.125
68 0.132571428571429
69 0.1915
70 0.0885714285714286
71 0.136
72 0.015
73 0.144
74 0.233333333333333
75 nan
76 nan
77 nan
78 nan
79 nan
80 nan
81 nan
82 nan
83 nan
84 nan
85 nan
86 nan
87 nan
88 nan
89 nan
90 nan
91 nan
92 nan
93 nan
94 nan
95 nan
96 nan
97 nan
98 nan
99 nan
100 nan
101 nan
102 nan
103 nan
104 nan
105 nan
106 nan
107 nan
108 nan
109 nan
110 nan
111 nan
112 nan
113 nan
114 nan
115 nan
116 nan
117 nan
118 nan
119 nan
120 nan
121 nan
122 nan
123 nan
124 nan
125 nan
126 nan
127 nan
128 nan
129 nan
130 nan
131 nan
132 nan
133 nan
134 nan
135 nan
136 nan
137 nan
138 nan
139 nan
140 nan
141 nan
142 nan
143 nan
144 nan
145 nan
146 nan
147 nan
148 nan
149 nan
150 nan
151 nan
152 nan
153 nan
154 nan
155 nan
156 nan
157 nan
158 nan
159 nan
160 nan
161 nan
162 nan
163 nan
164 nan
165 nan
166 nan
167 nan
168 nan
169 nan
170 nan
171 nan
172 nan
173 nan
174 nan
175 nan
176 nan
177 nan
178 nan
179 nan
180 nan
181 nan
182 nan
183 nan
184 nan
185 nan
186 nan
187 nan
188 nan
189 nan
190 nan
191 nan
192 nan
193 nan
194 nan
195 nan
196 nan
197 nan
198 nan
199 nan
200 nan
201 nan
202 nan
203 nan
204 nan
205 nan
206 nan
207 nan
208 nan
209 nan
210 nan
211 nan
212 nan
213 nan
214 nan
215 nan
216 nan
217 nan
218 nan
219 nan
220 nan
221 nan
222 nan
223 nan
224 nan
225 nan
226 nan
227 nan
228 nan
229 nan
230 nan
231 nan
232 nan
233 nan
234 nan
235 nan
236 nan
237 nan
238 nan
239 nan
};
\addplot [semithick, steelblue31119180]
table {%
0 0.12
1 0.0954285714285714
2 0
3 0.191428571428571
4 0.197857142857143
5 0.101
6 0.037
7 0.0484285714285714
8 0.100571428571429
9 0.0342857142857143
10 0.069
11 0.0468571428571429
12 0.191
13 0.0571428571428571
14 0.371
15 0.0468571428571429
16 0.2515
17 0.275428571428571
18 0.288
19 0.344
20 0.21
21 0.272
22 0.387
23 0.157714285714286
24 0.069
25 0.441142857142857
26 0.4575
27 0.106285714285714
28 0.374
29 0.198857142857143
30 0.657
31 0.457714285714286
32 0.5855
33 0.426857142857143
34 0.532
35 0.361142857142857
36 0.5535
37 0.305142857142857
38 0.184
39 0.913714285714285
40 0.835
41 0.729714285714286
42 0.7435
43 0.641714285714286
44 0.979
45 0.625142857142857
46 0.1245
47 0.392
48 0.665
49 0.633714285714286
50 0.9065
51 0.509142857142857
52 0.7325
53 0.782285714285714
54 0.9855
55 0.714857142857143
56 0.757
57 0.978857142857143
58 0.9455
59 0.449142857142857
60 1.0805
61 0.573142857142857
62 0.846
63 0.832
64 0.943
65 0.784571428571428
66 0.9605
67 0.974285714285714
68 1.1415
69 0.702857142857143
70 1.5145
71 0.74
72 1.3065
73 1.16057142857143
74 1.302
75 1.22914285714286
76 1.313
77 1.02514285714286
78 0.8705
79 1.11371428571429
80 1.098
81 0.548285714285714
82 1.2425
83 0.894785714285714
84 0.909928571428571
85 0.951
86 1.144
87 0.8465
88 1.22285714285714
89 1.089
90 1.43085714285714
91 1.0865
92 1.33028571428571
93 1.5945
94 1.26514285714286
95 1.432
96 1.33257142857143
97 1.127
98 0.908571428571429
99 1.55685714285714
100 nan
101 nan
102 nan
103 nan
104 nan
105 nan
106 nan
107 nan
108 nan
109 nan
110 nan
111 nan
112 nan
113 nan
114 nan
115 nan
116 nan
117 nan
118 nan
119 nan
120 nan
121 nan
122 nan
123 nan
124 nan
125 nan
126 nan
127 nan
128 nan
129 nan
130 nan
131 nan
132 nan
133 nan
134 nan
135 nan
136 nan
137 nan
138 nan
139 nan
140 nan
141 nan
142 nan
143 nan
144 nan
145 nan
146 nan
147 nan
148 nan
149 nan
150 nan
151 nan
152 nan
153 nan
154 nan
155 nan
156 nan
157 nan
158 nan
159 nan
160 nan
161 nan
162 nan
163 nan
164 nan
165 nan
166 nan
167 nan
168 nan
169 nan
170 nan
171 nan
172 nan
173 nan
174 nan
175 nan
176 nan
177 nan
178 nan
179 nan
180 nan
181 nan
182 nan
183 nan
184 nan
185 nan
186 nan
187 nan
188 nan
189 nan
190 nan
191 nan
192 nan
193 nan
194 nan
195 nan
196 nan
197 nan
198 nan
199 nan
200 nan
201 nan
202 nan
203 nan
204 nan
205 nan
206 nan
207 nan
208 nan
209 nan
210 nan
211 nan
212 nan
213 nan
214 nan
215 nan
216 nan
217 nan
218 nan
219 nan
220 nan
221 nan
222 nan
223 nan
224 nan
225 nan
226 nan
227 nan
228 nan
229 nan
230 nan
231 nan
232 nan
233 nan
234 nan
235 nan
236 nan
237 nan
238 nan
239 nan
};

\end{axis}
\node at (-1, 3.2)   (a) {(b)};
\end{tikzpicture}


==> sections/franka_task_result.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
tick align=outside,
tick pos=left,
title={Performance of algorithms on visual\_reacher},
x grid style={darkgray176},
xlabel={Time (min) },
xmin=-3.7, xmax=77.7,
xtick style={color=black},
y grid style={darkgray176},
ylabel={Average discounted Return},
ymin=-0.103645597242122, ymax=0.449061293762227,
ytick style={color=black}
]
\path [draw=steelblue31119180, fill=steelblue31119180, opacity=0.3]
(axis cs:0,0)
--(axis cs:0,0)
--(axis cs:1,0)
--(axis cs:2,-0.0032441449064852)
--(axis cs:3,-0.00711835253108848)
--(axis cs:4,0)
--(axis cs:5,-0.00437353232604107)
--(axis cs:6,0)
--(axis cs:7,-0.00700766889708519)
--(axis cs:8,-0.0133031897036116)
--(axis cs:9,-0.000381054071285095)
--(axis cs:10,-0.0173074961444431)
--(axis cs:11,-0.0023364337981084)
--(axis cs:12,-0.00199281896866585)
--(axis cs:13,0)
--(axis cs:14,0)
--(axis cs:15,0)
--(axis cs:16,-0.00739858546208276)
--(axis cs:17,-0.00352142402843841)
--(axis cs:18,-0.0273797765165357)
--(axis cs:19,-0.0126822662074169)
--(axis cs:20,-0.00368532332869659)
--(axis cs:21,-0.0169569369037319)
--(axis cs:22,-0.0131230824382654)
--(axis cs:23,0)
--(axis cs:24,0)
--(axis cs:25,-0.000395074329380621)
--(axis cs:26,-0.0410013286724646)
--(axis cs:27,-0.0181011369055651)
--(axis cs:28,-0.0484135424845029)
--(axis cs:29,-0.0477785944108411)
--(axis cs:30,-0.00772087433323646)
--(axis cs:31,-0.00221302629991356)
--(axis cs:32,0)
--(axis cs:33,-0.00262529086105303)
--(axis cs:34,-0.00343709427887415)
--(axis cs:35,-0.00829898229590038)
--(axis cs:36,0)
--(axis cs:37,0)
--(axis cs:38,-0.00193671534324986)
--(axis cs:39,-0.00835195502029722)
--(axis cs:40,0)
--(axis cs:41,-0.0175898804711963)
--(axis cs:42,-0.00872190135762144)
--(axis cs:43,-0.0239367215388698)
--(axis cs:44,-0.00580061208695875)
--(axis cs:45,-0.011613821079705)
--(axis cs:46,-0.0130404974131801)
--(axis cs:47,-0.012727497137599)
--(axis cs:48,-0.0127051545380548)
--(axis cs:49,-0.0108644218528203)
--(axis cs:50,-0.00231357780468401)
--(axis cs:51,-0.0218152751772231)
--(axis cs:52,-0.0105336849409104)
--(axis cs:53,-0.00300266476121019)
--(axis cs:54,-0.0219453380758903)
--(axis cs:55,0)
--(axis cs:56,-0.00446772405270945)
--(axis cs:57,-0.00936315570369058)
--(axis cs:58,-0.0227852811244438)
--(axis cs:59,-0.000985342370643506)
--(axis cs:60,-0.00301532267338968)
--(axis cs:61,0.0013099677520754)
--(axis cs:62,0.00219156110956452)
--(axis cs:63,-0.0118883162300628)
--(axis cs:64,0)
--(axis cs:65,-0.00634213807373513)
--(axis cs:66,-0.0138893339481946)
--(axis cs:67,-0.0094502466641568)
--(axis cs:68,-0.0164083444823375)
--(axis cs:69,-0.0422602615260573)
--(axis cs:70,-0.00580319146300361)
--(axis cs:71,-0.00945571552707263)
--(axis cs:72,-0.00145593919767671)
--(axis cs:73,-0.0140006965107724)
--(axis cs:74,0.00156999120632761)
--(axis cs:74,0.0722679095757929)
--(axis cs:74,0.0722679095757929)
--(axis cs:73,0.0770009314851439)
--(axis cs:72,0.0148709512028326)
--(axis cs:71,0.067573749125516)
--(axis cs:70,0.0625191436744319)
--(axis cs:69,0.130302473038677)
--(axis cs:68,0.0584676192399249)
--(axis cs:67,0.045099610151494)
--(axis cs:66,0.0866241331740757)
--(axis cs:65,0.01955492572735)
--(axis cs:64,0)
--(axis cs:63,0.0366556417093604)
--(axis cs:62,0.0415879152563982)
--(axis cs:61,0.0308754926079493)
--(axis cs:60,0.0163132942467791)
--(axis cs:59,0.00303813897615081)
--(axis cs:58,0.111723260549068)
--(axis cs:57,0.068414289472411)
--(axis cs:56,0.0407056669005535)
--(axis cs:55,0)
--(axis cs:54,0.0829058417251399)
--(axis cs:53,0.0155164872276645)
--(axis cs:52,0.0826728872678564)
--(axis cs:51,0.0672637651297711)
--(axis cs:50,0.00713353156444238)
--(axis cs:49,0.0660722271976545)
--(axis cs:48,0.0391742264923356)
--(axis cs:47,0.0392431161742635)
--(axis cs:46,0.112494057085104)
--(axis cs:45,0.0829413196417802)
--(axis cs:44,0.0607124527833594)
--(axis cs:43,0.0738048914115153)
--(axis cs:42,0.0268925291859995)
--(axis cs:41,0.0542354647861885)
--(axis cs:40,0)
--(axis cs:39,0.0257518613125831)
--(axis cs:38,0.00597153897502041)
--(axis cs:37,0)
--(axis cs:36,0)
--(axis cs:35,0.0255885287456928)
--(axis cs:34,0.0105977073598619)
--(axis cs:33,0.0139900177866735)
--(axis cs:32,0)
--(axis cs:31,0.00682349775806682)
--(axis cs:30,0.0399766790281749)
--(axis cs:29,0.14731733276676)
--(axis cs:28,0.149275089327217)
--(axis cs:27,0.0558118387921591)
--(axis cs:26,0.128343462880531)
--(axis cs:25,0.00121814584892358)
--(axis cs:24,0)
--(axis cs:23,0)
--(axis cs:22,0.0404628375179849)
--(axis cs:21,0.0522838887865066)
--(axis cs:20,0.0113630802634811)
--(axis cs:19,0.0761964746552428)
--(axis cs:18,0.0844209775926517)
--(axis cs:17,0.0356541563051114)
--(axis cs:16,0.0228123051747552)
--(axis cs:15,0)
--(axis cs:14,0)
--(axis cs:13,0)
--(axis cs:12,0.00614452515338637)
--(axis cs:11,0.0252968439303745)
--(axis cs:10,0.0533647797786996)
--(axis cs:9,0.00117491671979571)
--(axis cs:8,0.0410181682528025)
--(axis cs:7,0.0437193764962562)
--(axis cs:6,0)
--(axis cs:5,0.0220266823402213)
--(axis cs:4,0)
--(axis cs:3,0.0219482536375228)
--(axis cs:2,0.0347293834757604)
--(axis cs:1,0)
--(axis cs:0,0)
--cycle;

\path [draw=darkorange25512714, fill=darkorange25512714, opacity=0.3]
(axis cs:0,0.0417073162112901)
--(axis cs:0,-0.0135266971496076)
--(axis cs:1,-0.0192680287091093)
--(axis cs:2,0)
--(axis cs:3,0.00639941029594611)
--(axis cs:4,0.00240662109684853)
--(axis cs:5,-0.00897267302203007)
--(axis cs:6,-0.0064994507278901)
--(axis cs:7,-0.0111748337025825)
--(axis cs:8,-0.012845407507357)
--(axis cs:9,-0.0118081628205715)
--(axis cs:10,-0.0126514185335771)
--(axis cs:11,-0.00753093258337205)
--(axis cs:12,-0.0138439641874453)
--(axis cs:13,-0.00384019379616495)
--(axis cs:14,-0.0343430661878899)
--(axis cs:15,-0.00349619752520151)
--(axis cs:16,-0.037629821620151)
--(axis cs:17,-0.0154369910355366)
--(axis cs:18,-0.0537202858049485)
--(axis cs:19,0.00499699947146516)
--(axis cs:20,0.00159308333520245)
--(axis cs:21,-0.0176481833418894)
--(axis cs:22,0.00200066700838322)
--(axis cs:23,-0.0168743788011367)
--(axis cs:24,-0.00124353108746411)
--(axis cs:25,-0.00497320884293884)
--(axis cs:26,-0.0108508614402295)
--(axis cs:27,0.0018872608304019)
--(axis cs:28,-0.026887350449466)
--(axis cs:29,-0.0277781340852887)
--(axis cs:30,0.00335679159102728)
--(axis cs:31,0.0198237858655575)
--(axis cs:32,-0.0308255185067991)
--(axis cs:33,0.0113939890205024)
--(axis cs:34,0.00199813740727496)
--(axis cs:35,0.00456695587608816)
--(axis cs:36,-0.0400561220604872)
--(axis cs:37,0.004948905998659)
--(axis cs:38,-0.00392707565052548)
--(axis cs:39,-0.0785225567419242)
--(axis cs:40,0.012336847811674)
--(axis cs:41,0.0321561312509867)
--(axis cs:42,-0.0391312083905936)
--(axis cs:43,0.00779248699878909)
--(axis cs:44,0.0284813733949864)
--(axis cs:45,0.0247003026519961)
--(axis cs:46,0.0108575937778682)
--(axis cs:47,0.0272251464921417)
--(axis cs:48,0.0517048149329188)
--(axis cs:49,-0.0528921739134149)
--(axis cs:50,0.0257029811499503)
--(axis cs:51,-0.00734413214725899)
--(axis cs:52,0.0222349483124049)
--(axis cs:53,-0.052678914204983)
--(axis cs:54,0.0343169216460507)
--(axis cs:55,0.00926561614038884)
--(axis cs:56,-0.0217714020940024)
--(axis cs:57,-0.000492291183602195)
--(axis cs:58,-0.00277952001035722)
--(axis cs:59,0.0140805801354078)
--(axis cs:60,0.0314281850438623)
--(axis cs:61,0.0132080211492629)
--(axis cs:62,0.0118023888311514)
--(axis cs:63,0.00627057307120313)
--(axis cs:64,0.0604396139585349)
--(axis cs:65,0.0324781541800514)
--(axis cs:66,0.0276784735112061)
--(axis cs:67,0.0527126347771343)
--(axis cs:68,0.0681711960161763)
--(axis cs:69,0.0358530597312082)
--(axis cs:70,0.142235473972405)
--(axis cs:71,0.0369451195811774)
--(axis cs:72,0.088953990423153)
--(axis cs:73,0.0641673262847142)
--(axis cs:74,0.129884495800698)
--(axis cs:74,0.345803397656979)
--(axis cs:74,0.345803397656979)
--(axis cs:73,0.362383833988266)
--(axis cs:72,0.307972968902011)
--(axis cs:71,0.245788047469587)
--(axis cs:70,0.361170033395968)
--(axis cs:69,0.218711712880055)
--(axis cs:68,0.317667543963364)
--(axis cs:67,0.281689251347026)
--(axis cs:66,0.294553271096575)
--(axis cs:65,0.259558595640962)
--(axis cs:64,0.317569390169448)
--(axis cs:63,0.308948701071871)
--(axis cs:62,0.31870514222007)
--(axis cs:61,0.239990189743729)
--(axis cs:60,0.347928942808072)
--(axis cs:59,0.148311575878135)
--(axis cs:58,0.344082631424049)
--(axis cs:57,0.398533994885666)
--(axis cs:56,0.290580373790628)
--(axis cs:55,0.226085497485921)
--(axis cs:54,0.332317033695716)
--(axis cs:53,0.33005278032225)
--(axis cs:52,0.295938264272315)
--(axis cs:51,0.18449850636608)
--(axis cs:50,0.361716040138536)
--(axis cs:49,0.287675908332963)
--(axis cs:48,0.23419074640503)
--(axis cs:47,0.122134427264598)
--(axis cs:46,0.0731920414117444)
--(axis cs:45,0.279501109206055)
--(axis cs:44,0.327652018745942)
--(axis cs:43,0.198579339499544)
--(axis cs:42,0.35394043952646)
--(axis cs:41,0.223755353866659)
--(axis cs:40,0.321509369706647)
--(axis cs:39,0.42393825326203)
--(axis cs:38,0.0785580454188364)
--(axis cs:37,0.0961576375344086)
--(axis cs:36,0.237123662728647)
--(axis cs:35,0.118352975738435)
--(axis cs:34,0.206173471684284)
--(axis cs:33,0.142394395956551)
--(axis cs:32,0.276286966771636)
--(axis cs:31,0.175299275582073)
--(axis cs:30,0.233415174713262)
--(axis cs:29,0.126916922595429)
--(axis cs:28,0.136199102744943)
--(axis cs:27,0.0457973544707523)
--(axis cs:26,0.173776388409624)
--(axis cs:25,0.192018908375759)
--(axis cs:24,0.0120172404734017)
--(axis cs:23,0.0831775185977271)
--(axis cs:22,0.132900220197495)
--(axis cs:21,0.125989792500375)
--(axis cs:20,0.116020262126513)
--(axis cs:19,0.108772130983542)
--(axis cs:18,0.165637547898591)
--(axis cs:17,0.119940705543539)
--(axis cs:16,0.146218235015537)
--(axis cs:15,0.037627443619123)
--(axis cs:14,0.211085562980591)
--(axis cs:13,0.0279654340039739)
--(axis cs:12,0.0966981190559682)
--(axis cs:11,0.0253846510623358)
--(axis cs:10,0.0582579730811576)
--(axis cs:9,0.0364085020300956)
--(axis cs:8,0.0773378909542166)
--(axis cs:7,0.0439642600612341)
--(axis cs:6,0.0362302496515731)
--(axis cs:5,0.0893230325669292)
--(axis cs:4,0.117479113410919)
--(axis cs:3,0.0872594119586812)
--(axis cs:2,0)
--(axis cs:1,0.0594097551864204)
--(axis cs:0,0.0417073162112901)
--cycle;

\addplot [semithick, steelblue31119180]
table {%
0 0
1 0
2 0.0157426192846376
3 0.00741495055321717
4 0
5 0.00882657500709013
6 0
7 0.0183558537995855
8 0.0138574892745955
9 0.000396931324255307
10 0.0180286418171282
11 0.0114802050661331
12 0.00207585309236026
13 0
14 0
15 0
16 0.00770685985633621
17 0.0160663661383365
18 0.028520600538058
19 0.031757104223913
20 0.00383887846739228
21 0.0176634759413874
22 0.0136698775398598
23 0
24 0
25 0.00041153575977148
26 0.0436710671040332
27 0.018855350943297
28 0.0504307734213572
29 0.0497693691779595
30 0.0161279023474692
31 0.00230523572907663
32 0
33 0.00568236346281022
34 0.0035803065404939
35 0.00864477322489623
36 0
37 0
38 0.00201741181588527
39 0.00869995314614294
40 0
41 0.0183227921574961
42 0.00908531391418901
43 0.0249340849363227
44 0.0274559203482003
45 0.0356637492810376
46 0.0497267798359622
47 0.0132578095183323
48 0.0132345359771404
49 0.0276039026724171
50 0.00240997687987918
51 0.022724244976274
52 0.036069601163473
53 0.00625691123322716
54 0.0304802518246248
55 0
56 0.018118971423922
57 0.0295255668843602
58 0.044468989712312
59 0.00102639830275365
60 0.00664898578669473
61 0.0160927301800124
62 0.0218897381829814
63 0.0123836627396488
64 0
65 0.00660639382680743
66 0.0363673996129405
67 0.0178246817436686
68 0.0210296373787937
69 0.0440211057563097
70 0.0283579761057141
71 0.0290590167992217
72 0.00670750600257796
73 0.0315001174871857
74 0.0369189503910602
};
\addlegendentry{SAC}
\addplot [semithick, darkorange25512714]
table {%
0 0.0140903095308413
1 0.0200708632386556
2 0
3 0.0468294111273137
4 0.059942867253884
5 0.0401751797724496
6 0.0148653994618415
7 0.0163947131793258
8 0.0322462417234298
9 0.012300169604762
10 0.0228032772737902
11 0.00892685923948189
12 0.0414270774342614
13 0.0120626201039045
14 0.0883712483963504
15 0.0170656230469608
16 0.0542942066976928
17 0.0522518572540014
18 0.0559586310468213
19 0.0568845652275036
20 0.0588066727308576
21 0.054170804579243
22 0.0674504436029391
23 0.0331515698982952
24 0.00538685469296878
25 0.09352284976641
26 0.0814627634846974
27 0.0238423076505771
28 0.0546558761477387
29 0.04956939425507
30 0.118385983152145
31 0.0975615307238154
32 0.122730724132418
33 0.0768941924885268
34 0.104085804545779
35 0.0614599658072614
36 0.09853377033408
37 0.0505532717665338
38 0.0373154848841554
39 0.172707848260053
40 0.16692310875916
41 0.127955742558823
42 0.157404615567933
43 0.103185913249167
44 0.178066696070464
45 0.152100705929025
46 0.0420248175948063
47 0.0746797868783698
48 0.142947780668975
49 0.117391867209774
50 0.193709510644243
51 0.0885771871094105
52 0.15908660629236
53 0.138686933058634
54 0.183316977670883
55 0.117675556813155
56 0.134404485848313
57 0.199020851851032
58 0.170651555706846
59 0.0811960780067716
60 0.189678563925967
61 0.126599105446496
62 0.165253765525611
63 0.157609637071537
64 0.189004502063991
65 0.146018374910507
66 0.16111587230389
67 0.16720094306208
68 0.19291936998977
69 0.127282386305632
70 0.251702753684187
71 0.141366583525382
72 0.198463479662582
73 0.21327558013649
74 0.237843946728838
};
\addlegendentry{CTCO}
\end{axis}

\end{tikzpicture}

